Towards Trustworthy and Aligned Machine Learning: A Data-centric Survey with Causality Perspectives

The trustworthiness of machine learning has emerged as a critical topic in the field, encompassing various applications and research areas such as robustness, security, interpretability, and fairness. The last decade saw the development of numerous methods addressing these challenges. In this survey, we systematically review these advancements from a data-centric perspective, highlighting the shortcomings of traditional empirical risk minimization (ERM) training in handling challenges posed by the data. Interestingly, we observe a convergence of these methods, despite being developed independently across trustworthy machine learning subfields. Pearl's hierarchy of causality offers a unifying framework for these techniques. Accordingly, this survey presents the background of trustworthy machine learning development using a unified set of concepts, connects this language to Pearl's causal hierarchy, and finally discusses methods explicitly inspired by causality literature. We provide a unified language with mathematical vocabulary to link these methods across robustness, adversarial robustness, interpretability, and fairness, fostering a more cohesive understanding of the field. Further, we explore the trustworthiness of large pretrained models. After summarizing dominant techniques like fine-tuning, parameter-efficient fine-tuning, prompting, and reinforcement learning with human feedback, we draw connections between them and the standard ERM. This connection allows us to build upon the principled understanding of trustworthy methods, extending it to these new techniques in large pretrained models, paving the way for future methods. Existing methods under this perspective are also reviewed. Lastly, we offer a brief summary of the applications of these methods and discuss potential future aspects related to our survey. For more information, please visit http://trustai.one.

==> oldfiles/pretrained.tex <==
In the preceding sections, we have discussed the techniques and approaches of standalone models in the context of trustworthy machine learning. 
These models, though effective in their respective tasks, often require separate training for each new dataset and task, leading to potential inefficiencies and limitations. 
The emergence of pre-trained models has revolutionized the landscape of machine learning, particularly in natural language processing, 
by capitalizing on the vast knowledge gained from unsupervised pre-training on massive data.

This shift in paradigm towards pre-trained models and fine-tuning, also known as in-context learning, has not only streamlined the process of training models for specific tasks but has also resulted in significant improvements in performance across a wide range of applications. 
As we delve into pre-trained models, we will discuss various aspects of these models, including their architecture, training strategies, and fine-tuning techniques.

In the upcoming sections, we will explore how pre-trained models have transformed the field of machine learning and how they have contributed to the trustworthiness of machine learning systems. Throughout this discussion, it is essential to recognize the shared foundation between standalone and pre-trained models. Despite the differences in training methodologies, the core statistical techniques underlying pre-trained models remain similar to those used in standalone models.

By examining the statistical techniques and methodologies employed in both models, we can gain a deeper understanding of the factors contributing to machine learning systems' trustworthiness. In doing so, we aim to provide a comprehensive overview of trustworthy machine learning in the era of pre-trained models and in-context learning, building upon the foundation established through our examination of standalone models.

\subsection{Prompt-Tuning}

\subsubsection{Background}

\begin{equation}
    P(\y|\x) \approx f(\y|\mathcal{F}(\x);\theta)
\end{equation}


\paragraph{Chain of Thought Learning}


\paragraph{In-Context Learning}

Large language models (LMs) have gained the \emph{emergent abilities} \cite{?}
% Take citation from the paper of survey on llms
to predict particular tasks using sample inputs and other optional parameters, such as instructions ($\mathcal{I}$). 
For example, we can give a few examples of task sentiment analysis with input sentence and its label, i.e. positive or negative with the test input. 
What is particularly surprising is that LMs can achieve this prediction capability without optimizing their parameters. 
In other words, through in-context learning, LMs can utilize their existing trained weights to predict outputs for new tasks, providing an adequate number of samples and labels. 
Mathematically, the task can be defined using equation~\ref{eqn:incontext}.

\begin{equation} \label{eqn:incontext}
    P(\y|\x) \approx f(\y|\x, \{\x_i,\y_i\}_{i = 0}^{i = n}, \mathcal{I};\theta)
\end{equation}

Numerous studies have investigated and shed light on the factors that explain the ability of LMs \cite{?}, their limitations \cite{?}, and their dependency factors \cite{?} on this behavior. 
According to these studies, the emergent qualities of LMs can be attributed to the learning of concepts\footnote{It can be regarded as a latent variable that contains an inherent statistical relationship between different entities of various texts} during their training process via learning various concepts \cite{?}, \hwc{I told you a million times, stop worshiping things cannot be explained by statistics!}
% Shin et al. (2022a), Xie et al.(2022)
in other words, the training data consist of diverse corpora. 
The large size of LMs acts as another parameter, where they attain this ability as their size increases \cite{?}.
% Brown et al. (2020) also
The reasoning behind this behavior is explained by the work \cite{?}, which argues that LMs like GPT-3 (which was one of the early works to shed light on in-context learning) have similar architecture to transformers \cite{?}.
% Taken from the survey paper on llms
Furthermore, transformers are proven to have the ability to write linear models in their hidden state and they can update the linear model by implementing simple linear algorithms.
Hence, it proves that these models do not only retract the concepts from the training set but can also learn new tasks \cite{?}.

Apart from the reasons for emerging qualities in the training scenario, some methods improve the ICL ability of the LMs in the inference scenario, such as \emph{model warm-up}, and \emph{demonstration designing}.
Model warm-up acts as an intermediary fine-tuning stage between the pre-training and ICL inference stages.
Based on the aforementioned reasoning that a diverse corpus of pre-trained data improves ICL performance, \cite{?}
% (Chen et al., 2022a), Min et al. (2022b)
focuses to fine-tune the parameters of the LMs, making even small LMs perform better than large ones. 
Additionally, \cite{?}
% https://openreview.net/pdf?id=gEZrGCozdqR
adds that adding instructions while pre-training acts as a performance booster. 
On another hand, demonstration designing does not optimize the parameters of LMs but is data-driven, which includes formatting of input examples, or their selection. 
Many studies \cite{?} 
focus on selecting the examples, such that they have high information sharing
\cite{?} %Liu et. al 2022, rubin et al 2022
between them based on different metrics like distance or mutual information \cite{?}. %Sorensen et al 2022
Similarly, example order plays a crucial role in ICL performance \cite{?}
% Liu et al 2022
where the rightmost example should be highly similar to the input sample. 

\subsection{Parameter Efficient Fine-Tuning}

\mchry{We should fine-tune this section by binding it all using a master equation as done in all previous sections. Hence tuning/binding the whole text according to that equation.}

\subsubsection{Background}
Fine-tuning involves re-configuring the original network for a specific task. 
However, fine-tuning all parameters in a large language model is highly resource-intensive due to the exponential rise in the parameters from LMs like BERT \cite{devlin2018bert} with $350$ million parameters (released in $2018$) to GPT$-3$ \cite{brown2020language} containing $175$ billion parameters.
It is not feasible or cost-effective to train the entire language model from scratch for each task. 
As a result, a sub-field called ``Parameter-Efficient Fine-Tuning'' (PEFT) has emerged within the research community. 
This sub-field concentrates on methods that tackle the challenges of minimizing computational demands and eliminating the need to create and store new networks for every task.
These methods aim to save memory, training time, and computational overhead.
The community has proposed various ways \cite{hu2021lora,edalati2022krona, vucetic2022efficient, zaken2021bitfit, guo2020parameter, sung2021training, donahue2014decaf, houlsby2019parameter, wang2022adamix, liu2022few, sung2022lst, hu2023llm, pfeiffer2020mad, pfeiffer2020adapterfusion, ruckle2020adapterdrop}
% This will contain all the works in this section
to accomplish PEFT, lying on the foundation or reasoning to fine-tune the network by involving fewer parameters for updates during training. 
In essence, the challenge lies in identifying the optimal and minimal weights for fine-tuning the model.
Certain methods \cite{hu2021lora,edalati2022krona} 
% Insert the low-rank representation models.
attempt to address this by identifying the low-rank representation of current weights of LM model, and hence infusing them with the pre-trained weights as trainable parameters, while keeping the original weights frozen. 
Research \cite{aghajanyan2020intrinsic} supports this approach by considering pre-trained models as low-dimensional intrinsic models that can learn effectively even when projected onto a random subspace.

In addition to obtaining the low-rank representation for fine-tuning, certain studies \cite{vucetic2022efficient, zaken2021bitfit, guo2020parameter, sung2021training, donahue2014decaf} choose a direct approach to identify the most suitable parameters \cite{vucetic2022efficient, zaken2021bitfit, guo2020parameter, sung2021training}, and selectively fine-tune layers \cite{donahue2014decaf} of the model. 
For instance, \cite{zaken2021bitfit} focuses on refining the pre-trained language model by manually selecting specific parameters, such as the ``bias'' parameter.
However, this approach is model-specific and limited in its applicability to compressed models that lack adaptability and flexibility. 
On the other hand, \cite{vucetic2022efficient, guo2020parameter} adopt a model-agnostic approach by masking parameters during training. 
In \cite{vucetic2022efficient}, parameters are categorized as trainable or non-trainable, while \cite{guo2020parameter} masks parameters to determine their relevance during training. 
Conversely, \cite{sung2021training} argues that although these model-agnostic models possess certain advantages, they become computationally infeasible as they unravel important parameters throughout training.
Consequently, \cite{sung2021training} proposes pre-computing the crucial parameters to be fine-tuned during training using the Fisher Information.


Furthermore, several studies \cite{houlsby2019parameter, wang2022adamix, liu2022few, sung2022lst, hu2023llm, pfeiffer2020mad, pfeiffer2020adapterfusion, ruckle2020adapterdrop} have explored the incorporation of additional parameters into neural networks. 
These extra parameters can only be re-parameterized during the fine-tuning process while the existing weights remain unchanged. 
The concept of adapters \cite{houlsby2019parameter}  represents an early example in this category, where adaptive training layers are added within the transformer layer. 
Subsequent research \cite{wang2022adamix, hu2023llm, pfeiffer2020mad, pfeiffer2020adapterfusion, ruckle2020adapterdrop} has expanded on this concept to further improve the efficiency of fine-tuning. 
AdapterFusion \cite{pfeiffer2020adapterfusion}, for instance, focuses on addressing catastrophic forgetting during fine-tuning and multi-task learning. 
It accomplishes this by training multiple adapter modules for each task and utilizing a fusion module that combines these adapter modules in different proportions to tackle specific tasks. 
Building upon AdapterFusion, AdapterDrop \cite{ruckle2020adapterdrop} addresses memory inefficiency concerns by suggesting that existing adapter modules can be removed without significant performance loss in lower transformer layers.

Moreover, two other approaches, namely Adamix \cite{wang2022adamix} and Mad-X \cite{pfeiffer2020mad}, introduce multiple adapter modules within the transformer layer. 
Adamix improves upon the adapter method by incorporating multiple adapter layers, randomly selected for each forward pass, to enhance performance. 
Similarly, Mad-X incorporates three types of adapters in the transformer layers: language-specific, task-specific, and invertible adapter modules. 
Mad-X leverages an invertible adapter module for the same set of parameters to adapt both input and output representations, specifically language embeddings.
In addition to adapter methods, other techniques \cite{liu2022few, sung2022lst} also focus on introducing additional parameters for task-specific fine-tuning (PEFT).
Instead of using adapter layers, one approach \cite{liu2022few} adds parameters that amplify the activation function in the transformer layers based on the inferred task. 
On the other hand, Ladder side training \cite{sung2022lst} 
argues that adapter models are memory-inefficient. To address this, they propose attaching a separate side network, detached from the pre-trained model, after pruning the pre-trained network.
Lastly, \cite{hu2023llm} aims to balance the utilization of series \cite{houlsby2019parameter}, parallel \cite{pfeiffer2020mad}, and LoRa (Layer-wise Relevance Allocation) \cite{hu2021lora} techniques in an aggregated manner to optimize the model's performance for a specific task.


\subsection{Distillation}

